MLCommons Chakra: Advancing Performance Benchmarking and Co-design using Standardized Execution Traces

The fast pace of artificial intelligence~(AI) innovation demands an agile methodology for observation, reproduction and optimization of distributed machine learning~(ML) workload behavior in production AI systems and enables efficient software-hardware~(SW-HW) co-design for future systems. We present Chakra, an open and portable ecosystem for performance benchmarking and co-design. The core component of Chakra is an open and interoperable graph-based representation of distributed AI/ML workloads, called Chakra execution trace~(ET). These ETs represent key operations, such as compute, memory, and communication, data and control dependencies, timing, and resource constraints. Additionally, Chakra includes a complementary set of tools and capabilities to enable the collection, analysis, generation, and adoption of Chakra ETs by a broad range of simulators, emulators, and replay tools. We present analysis of Chakra ETs collected on production AI clusters and demonstrate value via real-world case studies. Chakra has been adopted by MLCommons and has active contributions and engagement across the industry, including but not limited to NVIDIA, AMD, Meta, Keysight, HPE, and Scala, to name a few.

==> additional_results.tex <==
% \FloatBarrier
\newpage
\section{Appendix: Additional Results}
\label{sec:additional_results}

% \begin{table*}[t]
%   \caption{Counts of key operations per GPU for a single epoch.}
%   \centering
%   \resizebox{2\columnwidth}{!}{%
%   \begin{tabular}{|l|c|l|cccc|c|cccc|}
%     \hline
%     \textbf{Model} & \textbf{GPUs} & \textbf{Parallelization} &
%       \multicolumn{4}{c|}{\textbf{Computation}} &
%       \multicolumn{5}{c|}{\textbf{Communication}} \\
%     \cline{4-7}\cline{8-12}
%     & & & GeMM & Attn & ElemWise & Others & P2P & AllReduce & All2All & AllGather & ReduceScatter\\
%     \hline
%     \multirow{3}{*}{\makecell[l]{GPT3 5B}} 
%       & 8  & TP=8, w/ SP             & 37,248 & 6,144 & 24,832 & 165,207 & 0   & 514   & 0   & 18,816 & 12,416 \\
%       & 8  & PP=8                     & 4,608  & 768   & 3,072  & 21,475  & 136 & 2     & 0   & 0      & 0     \\
%       & 8  & FSDP=8                   & 4,656  & 768   & 3,104  & 9,400   & 0   & 17    & 0   & 784    & 400    \\
%     \hline
%     \multirow{2}{*}{\makecell[l]{GPT3 175B}} 
%       & 32 & TP=32 w/ SP              & 36,960 & 6,144 & 24,640 & 88,573  & 0   & 130   & 0   & 18,528 & 12,320  \\
%       & 64 & TP=4, DP=2, PP=8, w/SP   & 9,216  & 1,536 & 3,072  & 26,615  & 67  & 67    & 0   & 4,683  & 3,078   \\
%     \hline
%     \multirow{3}{*}{\makecell[l]{Llama3 70B}} 
%       & 8  & TP=4, PP=2               & 24,576 & 4,096 & 12,288 & 46,080  & 130 & 2     & 0   & 12,416 & 8,320  \\
%       & 8  & TP=8                     & 49,536 & 8,192 & 24,832 & 85,634  & 0   & 16,897& 0   & 0      & 0     \\
%       & 16 & TP=4, PP=2, DP=2         & 12,288 & 2,048 & 6,144  & 23,054  & 65  & 4,161 & 0   & 16     & 16    \\
%     \hline
%     \multirow{2}{*}{\makecell[l]{Mixtral 8x7B}} 
%     & 8 & TP=2, EP=4               & 5912  & 1024   & 7751   & 16657  & 0  & 291     & 1024  & 1322      & 1122     \\
%       & 32 & EP=8, PP=4               & 1,920  & 256   & 512    & 11,028  & 16  & 2     & 512 & 9      & 9     \\
%       & 128& TP=4, EP=8, PP=4         & 1,920  & 256   & 512    & 10,801  & 16  & 131   & 512 & 659    & 531  \\
%     \hline
%     \multirow{1}{*}{\makecell[l]{Mixtral 8x22B}} 
%       & 32 & EP=8, TP=4               & 3,596  & 896   & 6,333    & 13,277  & 0  & 243     & 896 & 1,134      & 905      \\
%     \hline
%     \multirow{1}{*}{\makecell[l]{DeepSeek-MoE}} 
%       & 8  & EP=8                     & 27,456 & 896   & 6,784  & 46,938  & 0   & 18    & 1,728 & 23   & 23    \\
%       \hline
%       \multirow{1}{*}{\makecell[l]{DLRM}} 
%       & 8  & MP=8                     & 77 & 0   & 152  & 878  & 5   & 9   & 10 & 0   &  0     \\
%       \hline
%         \multirow{1}{*}{\makecell[l]{Resnet50}} 
%       & 2  & MP=2                     & 33 & 0   & 347  & 3263  & 0   & 15   & 0 & 0  & 0  \\
%     \hline
%   \end{tabular}
%   }
%   \label{tab:key_operations_comparison}
% \end{table*}

% \begin{table}[!t]
%   \caption{Deepseek-R1 inference simulation, different cluster size and parallel strategies}
%   \centering
%   \resizebox{\columnwidth}{!}{%
%   \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     \multirow{2}{*}{\diagbox{TP}{GPUs}}    & \multicolumn{3}{c|}{Prefilling} & \multicolumn{3}{c|}{Decoding}     \\
%     \cline{2-7}
%            & 16x32     & 8x64      & 4x128     & 16x32     & 8x64      & 4x128     \\
%     \hline
%      1     & 357.495   &  360.255  & 377.059   & 1006.680  &  1120.404 & 1195.683  \\
%      \hline
%      2     & 373.289   &  431.517  & 646.562   & 643.583   & 756.911   & 813.572   \\
%      \hline
%      4     & 180.834   &  195.016  & 248.261   & 362.799   & 401.736   & 508.196   \\
%      \hline
%      8     & 204.070   &  208.143  & 222.446   & 379.989   & 400.282   & 463.374   \\
%     \hline
     
%   \end{tabular}
%   }
%   \label{tab:astra_scaling_expr_table}
% \end{table}

% \TODO{Put all the contents here in a separate submission}


%\subsection{Hardware-in-the-Loop Emulation Study Details}

%\autoref{fig:hw-in-loop-cdf-ar-a2a-new} discusses the CDF for concurrent execution of two collective communicaitons (AllToAll and AllReduce) extended from the isolated . We observe that the mixing incurs a long-tail Flow Completion Time (FCT) distribution for All-to-All creating stragglers that increase overall Job Completion Time.


%\insertFigure{hw-in-loop-cdf-ar-a2a-new}{Mixing collectives results of CDF}{0.98}{-1em}{-1em}

% \subsection{Additional Simulation studies on ASTRA-sim Simulator}

\subsection{Inference System Scalability Analysis using ASTRA-sim}

In this experiment, we simulate the deepseek-R1 inference system~\cite{deepseekV3R1_inference_system_2025} under different parallelism strategy for the scalability of prefill and decode independently. We assume a system composed of 64x8 H100 DGX GPUs, and a global batch size of 2048. The system is partitioned into smaller clusters, ranging from four clusters with 128 GPUs, to 16 clusters with 32 GPUs each, with the batch size divided proportionally across clusters.We vary two parallelism axes in our experiments: 1) EP/DP, where we do expert-parallel for routed experts and data-parallel for remain layers, 2) TP, where we apply tensor-parallel for all layers. We separate prefilling and decoding stages as they may prefer a different system, where prefilling has a sequence length of 1K, and decoding has a KV cache of 64K tokens.

~\autoref{tab:astra_scaling_expr_table} shows the end-to-end runtime of each system and parallel strategies. The EP/DP can be calculated by dividing cluster size and TP. From the results we can observe two points: 1) For either prefilling or decoding, appropriately increase tensor-parallel can reduce runtime, as it equivalently increase batch size and improve operational intensity. However, excessive tensor-parallelism introduces significant communication overhead compared to EP/DP, which can offset or even hide the potential speedup. 2) For prefilling stage, the system scale do not affect the runtime much, while decoding is more sensitive to system scale. Under the long-context decoding, a larger system results in a longer runtime. 

\begin{table}[!t]
  \caption{Deepseek-R1 inference simulation, different cluster size and parallel strategies}
  \centering
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\diagbox{TP}{GPUs}}    & \multicolumn{3}{c|}{Prefilling} & \multicolumn{3}{c|}{Decoding}     \\
    \cline{2-7}
           & 16x32     & 8x64      & 4x128     & 16x32     & 8x64      & 4x128     \\
    \hline
     1     & 357.495   &  360.255  & 377.059   & 1006.680  &  1120.404 & 1195.683  \\
     \hline
     2     & 373.289   &  431.517  & 646.562   & 643.583   & 756.911   & 813.572   \\
     \hline
     4     & 180.834   &  195.016  & 248.261   & 362.799   & 401.736   & 508.196   \\
     \hline
     8     & 204.070   &  208.143  & 222.446   & 379.989   & 400.282   & 463.374   \\
    \hline
     
  \end{tabular}
  }
  \label{tab:astra_scaling_expr_table}
\end{table}


\subsection{Detailed Simulation studies on Scala Computing Platform}

The Scala Compute Platform (SCP) is a high-performance commercial discrete-event simulator developed by Scala Computing and built on ns-3. SCP is used by data center operators and networking equipment manufacturers to perform large-scale Chakra simulations. It runs on on-demand compute clusters in the AWS cloud and supports simulations involving over 100,000 GPUs communicating via RoCEv2 or an enhanced Ethernet Transport (eET) inspired by the Ultra Ethernet Transport (UET) specs~\cite{ultra-ethernet}.

\noindent\textbf{Simulation Sytem.}The simulation is conducted on a system consisting of 256 GPUs. The network topology employs fully provisioned 51.2-Tb/s Ethernet switches organized in a two-tier Clos configuration, featuring 800-Gb/s inter-switch links and 400-Gb/s NICs. The workload is generated using Chakra traces synthesized with a STAGE~\cite{stage}, configured with model dimensions of $d_{\mathrm{in}} = d_{\mathrm{out}} = d_{\mathrm{model}} = 5120$, feed-forward dimension $d_{\mathrm{ffn}} = 13824$, sequence length $8192$, $40$ attention heads, and $80$ stacked transformer layers.
To estimate the computation times for this generated Chakra graphs, it is augmented with NVIDIA A100 profiling data. Workload parallelization is configured as 64 DP × 2 TP × 2 PP × 1 SP. The RDMA transport protocols evaluated include RoCEv2 and eET. Each simulation runs for a duration of 2 seconds and is executed on Scala’s MPI-enhanced ns-3 environment deployed on AWS.


% \insertFigure{what_if_network_bw_dgx}{Communication Time for Different Network Topology and Bandwidth - Mixtral 8x7B}{0.98}{-1em}{-1em}


\subsubsection{Overview}


We simulated an LLM workload on a small, two-tier RDMA network with 256 NVIDIA A100 GPUs. The study evaluated the workload’s performance over RoCEv2 and eET. For RoCEv2, the network was made “lossless” by enabling PFCs. For eET, PFCs were disabled and congestion was managed using NSCC and flow control, both inspired by UET. In addition, eET employed packet spraying with a 128-way spray size. 

A critical feature of LLM workloads is their high degree of synchrony: performance is strongly influenced by within-GPU dependencies between computation and communication operations, as well as cross-GPU dependencies (e.g., \texttt{SEND}/\texttt{RECEIVE}). Chakra’s ability to capture these dependencies is essential for accurate simulation of LLM workloads.

\subsubsection{Analysis and Metrics}
The metrics in this study include: (i) the distribution of NIC transmit–link utilization, (ii) aggregated NIC receive throughput, (iii) RTTs, (iv) congestion statistics and plots for PFC and NSCC, and (v) workload progress toward completion measured by the CDF of send bytes. For detailed analysis of (iii), (iv) and (v), it is included in the appendix attached with this submission.

\subsubsection{NIC Transmit/Receive Link Utilization}
The distribution of NICs by transmit utilization is shown in the \emph{Tx link utilization} heatmap \autoref{fig:SCALA_UET_NIC_RX_TX}(a) and \autoref{fig:SCALA_RoCE_NIC_RX_TX}(a). 
The y-axis reports utilization percentage, and the x-axis shows simulation time. Color encodes the count of NICs at each utilization level, with dark red indicating the maximum (256) and dark blue indicating zero. Notably, after 300\,ms for RoCEv2 and 500\,ms for eET, a large fraction of NICs are no longer transmitting at high rates. This arises from the synchronous nature of LLM workloads: prolonged intervals of low network utilization reflect GPUs spending substantial time on computation rather than communication (due to the nature of more DP than TP and PP in the experiment setup) or waiting to receive data from other GPUs.

Considering the receive-side NICs, we observe oscillatory behavior driven by the workload structure \autoref{fig:SCALA_UET_NIC_RX_TX}(b) and \autoref{fig:SCALA_RoCE_NIC_RX_TX}(b). Even with a fully provisioned topology, the average link utilization remains well below the 400\,Gb/s line rate, with extended periods of underutilization while GPUs are computing or waiting on dependencies.

\insertFigure{SCALA_UET_NIC_RX_TX}{Results of eET v2 NIC Transmit Receive}{0.98}{-1em}{-1em}

%\insertFigure{SCALA_RoCE_NIC_RX_TX}{Results of RoCE v2 NIC Transmit Receive}{0.98}{-1em}{-2em}
% \begin{figure*}[htbp]
%     \centering
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/Scala_ROCE_NIC_Tx_Link_Utilization.png}
%         \caption{ROCEv2}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/Scala_UET_NIC_Tx_Link_Utilization.png}
%         \caption{UET}
%     \end{subfigure}
%     \caption{Transmit Link Utilization}
% \end{figure*}



% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/Scala_ROCE_NIC_Aggregated_NIC_Rx_Throughput.png}
%         \caption{ROCEv2}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/Scala_UET_Aggregated_NIC_Rx_Throughput.png}
%         \caption{UET}
%     \end{subfigure}
%     \caption{Aggregated NIC Rx Throughput}
% \end{figure*}

\subsubsection{Round Trip Times}
RTT traces for both RoCEv2 and eET show periodic peaks, indicating congestion in the network. Although mean RTTs are low, RoCEv2 exhibits significantly higher peaks, above 1\,ms, whereas eET peaks are around 25\,\textmu s \autoref{fig:RTT}. This is consistent with UET NSCC aggressively keeping switch buffers shallow, whereas RoCEv2 relies on PFCs. Higher tail latencies can degrade the performance of tightly synchronized workloads such as LLMs.

\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Scala_UET_RTT.png}
        \caption{eET RTT}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Scala_ROCE_RTT.png}
        \caption{RoCE RTT}
    \end{subfigure}
    \caption{eET and RoCE RTT (with Mean and Max)}
    \label{fig:RTT}
\end{figure*}







\subsubsection{RoCE PFC Statistics}
PFC statistics indicate a significant number of pause frames \autoref{fig:PFC_stats}. Combined with RTT peaks, this substantiates periodic congestion in the RoCEv2 network. Considering that the network is fully provisioned and overall link utilization is low, the presence of congestion may seem puzzling at first. The workload structure explains it: only a limited subset of GPUs transmits at line rate at any given time, and RoCEv2 does not employ packet spraying, so it cannot fully exploit redundant paths. Occasional incasts and ECMP hotspots further contribute to the observed congestion.

% \TODO{shouldn't be a subfigure?}
% {\color{red}
% Mehryar: I was not sure if we had room to include a PFC plot, so to keep things brief I only included an overview "PFC Statistics" table which is currently labeled as Figure 18. However, if deemed beneficial, please feel free to include the file SCALA\_ROCE\_PFC\_Plot.png, which you will find in the "figures" subdirectory (though not included in the paper). The plot shows further detail beyond the "PFC Statistics" table, and shows at which point in the simulation the NICs were experiencing congestions (PFC XOFFs).
% }

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/SCALA_ROCE_PFC_Plot.png}
        \caption{Congestion of ROCE PFC along with Timeline}
    \end{subfigure}
    \caption{PFC Statistics}
    \label{fig:PFC_stats}
\end{figure}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Scala_ROCE_PFC_Statistics.png}
        \caption{ROCEv2}
    \end{subfigure}
    \caption{PFC Statistics}
    \label{fig:PFC_stats}
\end{figure}

\subsubsection{eET NSCC Congestion Control}
For the eET transport, we observe a number of ECN M-marked packets, indicating occasional congestion \autoref{fig:congestio_control}. To manage this congestion, eET NSCC reduces the congestion window, as shown in the violin plot of eET congestion-window size. Despite these episodes of network congestion, NSCC appears effective at keeping RTT to a mean below 5 microseconds and a maximum below 26 microseconds throughout the run (see the eET RTT plot). Keeping network latency low is crucial for improving the performance of highly synchronized workloads such as LLMs on scale-out networks.

\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Scala_UET_M_Marked_Packets_Received.png}
        \caption{eET ECN M-Marked Packets}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Scala_UET_Congestion_Window.png}
        \caption{eET Congestion Window}
    \end{subfigure}
    \caption{eET NSCC Congestion Control}
    \label{fig:congestio_control}
\end{figure*}

\subsubsection{CDF for Send Bytes simulating NVIDIA A100}
The send-bytes cumulative distribution function (``Send Bytes CDF'') plots show the progression of the simulation within the allotted two-second time limit (shown in \autoref{fig:send_byte-A100}). Because the simulation time was capped at two seconds, the run ended before all Chakra traces finished executing. For RoCEv2, the CDF indicates that 7.84\% of the workload’s total bytes were sent; for eET, 7.96\% were sent. Thus, despite eET’s performance enhancing features relative to RoCEv, such as 128\hyp{}way sprays and lower tail latency achieved via eET NSCC versus RoCEv2 PFC, these did not translate into a net performance improvement for eET in this particular simulation. This may seem counterintuitive at first, but further analysis shows that the bottleneck was not network communication; rather, computation on the GPUs limited overall workload performance.

\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Scala_ROCE_CDF.png}
        \caption{ROCEv2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Scala_UET_CDF.png}
        \caption{eET}
    \end{subfigure}
    \caption{Send Bytes Cumulative Distribution Function - A100}
    \label{fig:send_byte-A100}
\end{figure*}

\subsubsection{CDF for Send Bytes on Infinitely Fast GPU}
To validate that computation (not inter-GPU communication) is the limiting factor, we reran the simulation with all computation nodes’ \texttt{microDurations} attribute in the Chakra traces set to zero (shown in \autoref{fig:send_byte_infini}). This repeats the simulation under the assumption of an infinitely fast GPU that takes zero time to execute the computation nodes embedded in each Chakra trace. This assumption corresponds to an asymptotic case that we approach as we move from A100 to H100 to H200 and beyond. Under this assumption, we observe major differences between the performance of RoCEv2 and eET. In the RoCEv2 case, 17.4\% of the workload completed in two seconds. eET was significantly faster: 21.7\% of the workload completed in the same two seconds. These results validate that computation is indeed the performance-limiting factor.

Examining the CDF plots for the A100, two regions are apparent. In the initial region, before the simulation time reaches 300\,ms for RoCEv2 and 500\,ms for eET, the workload completes at a faster rate. Thereafter, execution slows markedly as the simulation enters a regime in which computation plays a larger role, reducing the likelihood that the network is the bottleneck. This slowdown is not observed when simulating an infinitely fast GPU: the workload’s send-bytes metric progresses with a nearly constant, single slope.

\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Scala_ROCE_Baseline_CDF.png}
        \caption{ROCEv2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Scala_UET_Baseline_CDF.png}
        \caption{eET}
    \end{subfigure}
    \caption{Send Bytes Cumulative Distribution Function - Infinitely Fast GPU}
    \label{fig:send_byte_infini}
\end{figure*}

\subsubsection{Key Takeaways}
\begin{itemize}
  \setlength{\itemsep}{2pt}   % space between items
  \setlength{\parsep}{0pt}    % extra paragraph space within items
  \setlength{\parskip}{0pt}   % paragraph skip (often already 0)
  \setlength{\topsep}{0pt}    % space above/below the list
  \item LLM workloads are highly synchronized; execution speed depends not only on the transport protocol but also on the workload’s fine-grained structure and the interplay between communication and computation tasks.
  \item Given the nature of LLM workloads, RDMA transports that achieve lower latency or exploit redundant network paths generally perform better, so long as computation is not the bottleneck. 
  \item Chakra provides an effective way to capture dependencies within and across GPUs, enabling fine-grained simulation of LLM workloads over RDMA.
  \item Large-scale (100k+ GPU) network simulators enabled by Chakra, such as the Scala Computing platform, allow investigation of LLM workloads at scale and help identify performance bottlenecks in workload design and transport, yielding substantial savings in AI training and inference.
\end{itemize}




==> background.tex <==
\section{Background and Motivation}

\TK{As we discussed, this section could perhaps now get removed as we already have everythng in intro}
\ju{May be we can alternate this section with itemized contributions at the end of intro section.}
%\TK{TODO}\ch{expand it}
% The importance of HW-SW codesign in designing distributed ML systems is well-known. Despite its importance, the necessary infrastructure for effective implementation remains insufficient. Three primary challenges hinder progress in this area. Firstly, the absence of a unified schema for exchanging execution traces of ML models poses a significant obstacle. Although numerous ML frameworks and languages exist, their primary focus has been on representing and optimizing ML models, with performance modeling receiving less attention. Consequently, no standard schema for encoding execution information has been developed. Secondly, the lack of toolchains for performance modeling is another challenge. Comprehensive toolchains are crucial for identifying bottlenecks and debugging issues efficiently. Lastly, sharing traces across organizations and researchers remains difficult due to proprietary constraints. Traces obtained from real executions and, when needed, synthetic traces that preserve key execution characteristics enable safe exchange and support performance projection for systems with varying system sizes and interconnect configurations.

Distributed ML systems are inherently complex and call for coordinated efforts from both hardware and software. The importance of hardware-software co-design in achieving performant, efficient, and scalable distributed ML is well-known. Despite its importance, the necessary infrastructure to search for effective implementation remains insufficient. Three primary challenges hinder progress in this area.

\JY{Ground with, e.g. company 1 uses this, company 2 uses this, etc. Not much need for broad background section. It's just straightforward. Copy/paste to intro. If you say 'lack of unified schema', what are the examples, of different/fragmented schemas.}

\noindent\textbf{Lack of unified schema.} The lack of a unified schema for exchanging execution traces of machine learning workloads is a major challenge for conducting system performance analysis and co-design. Over the years, many ML frameworks have been developed and successfully used in different scenarios and applications. However, the transferability between different frameworks often becomes a problem, as each framework usually have its own schema of execution traces. The fragmentation creates barriers to platform-agnostic system-level analysis and co-design, and limits the opportunities for cross-platform optimizations. As a result, system-level optimizations are often limited to the boundaries of individual frameworks, restricting broader collabration and innovation.

\noindent\textbf{Lack of performance modeling toolchain.}  Comprehensive toolchains are crucial for identifying bottlenecks and debugging issues efficiently. Although powerful performance modeling tools exist,
% for example, NVIDIA nSight\cite{} and PyTorch Kineto \cite{}, 
they are mostly focused on single-node profiling instead of the whole distributed ML system. The lack of system-level performance modeling tools makes it difficult to understand the interactions and dynamics of distributed ML systems as a whole, which limitation is particularly crucial for designing and optimizing scalable distributed ML systems, especially where insights into cross-node perforamnce are necessary to guide hardware and softward decisions.

% \ch{If we claim this point, we need to show the ability that we can hidden those system details, while performance-wised char still keeped?}
\noindent\textbf{Trace sharing challenges.} Sharing traces across organizations and researchers remains difficult due to proprietary constraints. Many organizations consider detailed execution data to be sensitive proprietary information, as it may expose internal model architectures, parallelization and optimization strategies, and hardware configurations. As a result, research and system designers often cannot access or exchange traces freely, and are limited to open-source implementations. This reliance on open-source implementations may alienate researchers from characteristics real-world production workloads, limiting the ability of their analysis and optimizations. In conclusion, the lack of access to realistic, diverse execution traces makes it difficult to develop relevant system-level optimizations and slows innovation in distributed ML system design.



==> camera-ready-revision.tex <==
\section{Camera Ready Revision Plan}
We thank the reviewers once more for their feedback and accepting our submission. We have outlined our plans to incorporate the reviewers' feedback for the camera ready version. 


\subsection{Representing modern techniques and deployments}
We will add the following discussion and studies to showcase how Chakra can capture LLM-era techniques and deployments. \textcolor{red}{New additions are highlighted in red in \autoref{sec:inference_analysis}. and partially in \autoref{sec:post-exec-trace}}

\begin{enumerate}
    \item Sparse MoE Routing:
    
    Unlike training frameworks such as NeMo, which drop or pad tokens to balance all-to-all communication, inference uses sparse MoE routing that keeps every input token. So far we have not collected Chakra traces from inference workloads using sparse MoE, but will generate, collect, and discuss such traces in our camera ready version. We will first come up with a  schema (\textit{reuse or extend the existing ones in \autoref{tab:chakra-comm-schema}}) to represent the imbalanced message volume between src-dst pairs. Next, we will add the mechanism in vLLM to profile the per-message volume. (This task is required to generate Chakra traces from real systems as discussed in \autoref{sec:post-exec-trace}, and is not required in the synthetic approach in \autoref{sec:pre-exec-trace}.) The resulting Chakra traces will reflect token-to-expert distributions that occur in real deployment.
    
    \item Multi-tier memory offloading:
    
    To demonstrate Chakra’s capability to capture and analyze memory offloading, we will add an experiment comparing Chakra traces generated with offloading enabled to those generated without it. From the Chakra traces, we will extract Chakra nodes corresponding to 'CPU-to-GPU transfer' operations. These Chakra nodes are embedded with the transfer duration, which captures the contention induced by concurrent offloaded accesses.
    
    \item KV-Cache Transfer:

    Similar to the Sparse MoE routing, we do not have traces showing KV Cache transfer, but will collect and discuss these traces for the camera ready version. We will add the mechanism to profile the message size of the point-to-point message that transfers the KV Cache between prefill and decode GPUs.The Chakra nodes captured can annotate the information about KV Cache size and the communicating GPU pairs using existing schema parameters, similar to Pipeline Parallelism.

\end{enumerate}

To achieve the above analysis, we use the following two main approaches depending on real-system accessibility and availability. (a) A trace-driven approach that converts execution traces collected from real systems into Chakra traces (\autoref{sec:post-exec-trace}). (b) A synthetic approach that generates Chakra traces using hardware-specific parameters and explicit dependencies to approximate real system behavior (\autoref{sec:pre-exec-trace}). 
% Expand discussions for the following:
% Table 3 shows the per-operator tensor format on a single device. Offloading and remote-access operations can be modeled as individual Chakra nodes (Table 2), with appropriate data and control dependencies to explicitly annotate the corresponding data movement.

\subsection{Motivation and shortcoming of related work}

Given the extra 2 pages for camera-ready version, we will expand the discussion for related work based on the context in the appendix A. We will emphasize the lack of holistic tracing for distributed AI, why this is important, and highlight the fact that Chakra addresses this demand 
\textcolor{red}{New additions are highlighted in red in \autoref{sec:related_work}.}

\subsection{Lessons Learned}
In addition to expanding the related work, we will add further details on future directions and ongoing efforts informed by lessons learned across different stages of development. This discussion will be based on the following rebuttal response (copied verbatim). \textcolor{red}{New additions are highlighted in red in \autoref{sec:lessons_learned_extensions}.}

Here are some of the lessons we learned while working with Chakra:
\begin{itemize}
\item A graph-based execution trace (ET) effectively bridges the gap between high-level frameworks (e.g. PyTorch), LLM frameworks (e.g. Nemo), and downstream replay/simulation tools; help provide a common abstraction from multiple industry participants to exchange critical bottlenecks without revealing sensitive IP.
\item By abstracting execution into compute, memory, and communication nodes with explicit dependencies, we can enable portable and reproducible benchmarking without disclosing model weights or datasets. This has allowed Meta/NVIDIA to identify bottlenecks in overlapping compute/comms that were invisible in isolated benchmarks \cite{saeed_enable_2021}.
\item Our experience reaffirms a cyclic process from productive SW/HW codesign: observe (in production) $\rightarrow$ reproduce (via replay) $\rightarrow$ design/evaluate new solutions (via simulators) $\rightarrow$ deploy (in production). To summarize, Chakra acts as the standardized mechanism for representing key performance aspects of a workload through every stage of the co-design cycle.
\end{itemize}


% \subsection{Reviewers' Feedback}

% Reviewers saw it as a valuable industry contribution with real community effort behind it. It offers practical, end-to-end systems lessons (including operational/governance aspects) that many practitioners and students may not be aware of, and provides enough implementation detail to be useful to typical ML systems readers.

% The main gap is generality vs. modern practice. The paper should add a clear discussion of how the framework would (or wouldn’t) represent newer LLM-era patterns—e.g., disaggregated prefill/decode, KV-cache lifetime/ownership and offload across memory tiers, parameter sharding, sparse MoE routing, and resource contention/queuing. The goal is to acknowledge what would require extensions and what can be captured faithfully today, without claiming “it can be modeled” without precision.


==> generative_model.tex <==
% % TK: I changed generation to collection
% \section{ET collection and synthesis}

% Collecting all production traces data on a regular cadence is feasible with the tooling support provided by Chakra. However, due to the massive amount of data, it is not scalable or effective to replay all of them for benchmarking. Additionally, sharing these traces may not be advised since it would be possible to reconstruct the original model. This could result in proprietary model information being shared widely. Therefore, automatically discovering a representative set of traces is crucial to complete the whole system. To address this issue, we propose a methodology for generating representative traces using generative machine learning models based on production trace data.

% Our approach enables efficient generation of realistic-looking production and futuristic traces, which can be used for data-driven decision making. Furthermore, it provides representative traces as the single source of truth that can be shared internally and externally given the stochastic nature of the generative models, which naturally provides an obfuscation of the production data. We start our modeling work from analyzing the communication part of the trace, the same framework can be easily extended to full trace.

% The communication part of the traces contains communication collectives across a set of GPUs (ranks). There are a few hard constraints on the traces within the same process group to ensure the replay system can run these traces without raising errors. To better address these constraints, we propose a concept of “master trace”, which is a lossless compression of all $N$ traces of all ranks taking all constraints into consideration. We can construct a master trace from $N$ traces of all ranks, and reconstruct $N$ traces from this master trace without losing any information. The master trace helps us to learn a distribution and synthesize traces without worrying about violating the constraints of the replay system.

% Based on the master trace data, we developed a hierarchical ML model comprising several generators that ensure the synthesized traces follow the expected data distributions. See \autoref{fig:genai_model} for an overview of this model. There are a couple of advantages for the hierarchical model that facilitates model research and experimentation. It is modularized and flexible. We can substitute the individual generator parts with various algorithms. We can easily extend the model with additional generation stages when needed. This facilitates model research and experimentation. It is also interpretable and easy for debugging. The model is conceptually easy to understand. Even when we use complex algorithms for the generators, we are able to evaluate performance at each stage and identify bottlenecks for improvements. This is a big advantage for model debugging and interpretation compared to a single blackbox model where debugging is difficult. Moreover, the model of generators follow the actual param trace generation logic. It provides us data insights into the param trace generation stages, enabling deeper understanding of param trace patterns.

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.98\columnwidth]{figures/genai_model.png}
%     \\
%     \caption{Generative AI model for ET synthesis.}
%     \label{fig:genai_model}
% \end{figure}

% For network use cases, the composition of collective types and the message sizes are the key factors. The Comm Type Generator ensures that the generated collective types align with the collective composition of production traces. We have identified two major clusters of collective type compositions. The Message Size Generator ensures that the message size generated follows the distribution of each collective type. We developed Gaussian mixture models to fit the data and draw samples from the fitted distribution. The synthesized samples align relatively well with the true distribution. We have modeled the distributions of comm types, comm sequence length, GPU sizes, message sizes, autocorrelation between comm types and message sizes, and message splits across GPUs, as well as the dependencies between the generators. We have tested the synthesized traces using the replay system and found that they work correctly on our training cluster. 

% The generative models can be extended to generate traces for larger futuristic system scales and compute \& communication traces, which will capture compute-communication overlap, dependency structure, etc. Overall, our generative AI models enables efficient generation of representative traces, which will be a valuable tool for optimizing distributed AI training and evaluating future hardware designs.

==> include/cmds.tex <==
\makeatletter
% Render the list of affiliations as a centered inline block, intended
% to be placed directly below the author list (inside the title block).
\newcommand{\printAffiliationsBox}{%
  \begin{center}
    \small
    \stepcounter{@affiliationcounter}%
    \setcounter{@affilnum}{0}%
    \forloop{@affilnum}{1}{\value{@affilnum} < \value{@affiliationcounter}}{%
      \textsuperscript{\arabic{@affilnum}}%
      \ifcsname @affilname\arabic{@affilnum}\endcsname
        \csname @affilname\arabic{@affilnum}\endcsname
      \else
        {\bf AUTHORERR: Missing \textbackslash{}mlsysaffiliation.}%
      \fi
      \hspace{0.9em}%
    }%
    \addtocounter{@affiliationcounter}{-1}%
  \end{center}
}
% Print the notice (and correspondence) as a first-column footnote,
% without re-listing the affiliations.
\newcommand{\printNoticeOnly}[1]{%
  {\let\thefootnote\relax\footnotetext{\hspace*{-\footnotesep}%
    \ifdefined\isaccepted #1\fi%
    \ifdefined\mlsyscorrespondingauthor@text
      Correspondence to: \mlsyscorrespondingauthor@text.%
    \else
      {\bf AUTHORERR: Missing \textbackslash{}mlsyscorrespondingauthor.}%
    \fi
    \ifx\Notice@String\@empty\else
      \ \\
      \Notice@String
    \fi
  }}%
}
\makeatother

\newcommand{\Chakraet}{\texttt{Chakra ET}\xspace}
\newcommand{\ptet}{\texttt{PT ET}\xspace}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,fill,inner sep=0.7pt] (char) {\textcolor{white}{#1}};}}

\renewcommand{\UrlFont}{\ttfamily\footnotesize}


\renewcommand{\lstlistingname}{Snippet}
\renewcommand{\sectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Section}

\newcommand{\TODO}[1]{\textcolor{red}{[\textbf{TODO}]}{\textcolor{red}{\xspace\textbf{#1}}}}
\newcommand{\fixme}{\textcolor{red}{FIXME}}
\newcommand{\placeholder}[1]{\textcolor{lightgray}{#1}}
\newcommand{\tkheo}[1]{\textcolor{blue}{Taekyung:}{\textcolor{orange}{\xspace#1}}}
\newcommand{\TK}[1]{\textcolor{blue}{Tushar:}{\textcolor{orange}{\xspace#1}}}
\newcommand{\SR}[1]{\textcolor{blue}{Srinivas:}{\textcolor{orange}{\xspace#1}}}
\newcommand{\ZW}[1]{\textcolor{blue}{Zhaodong:}{\textcolor{orange}{\xspace#1}}}
\newcommand{\ju}[1]{\textcolor{blue}{[Joongun:]}{\textcolor{orange}{\xspace#1}}}
\newcommand{\HX}[1]{\textcolor{blue}{[Huan:]}{\textcolor{orange}{\xspace#1}}}
\newcommand{\HW}[1]{\textcolor{blue}{[Hanjiang:]}{\textcolor{orange}{\xspace#1}}}
\newcommand{\WL}[1]{\textcolor{blue}{[Winston:]}{\textcolor{orange}{\xspace#1}}}
% \newcommand{\WW}[1]{\textcolor{blue}{[William:]}{\textcolor{orange}{\xspace#1}}}
\newcommand{\VR}[1]{\textcolor{blue}{[Vijay:]}{\textcolor{orange}{\xspace#1}}}
\newcommand{\DK}[1]{\textcolor{blue}{[David:]}{\textcolor{orange}{\xspace#1}}}
\newcommand{\MG}[1]{\textcolor{blue}{[Mehryar:]}{\textcolor{orange}{\xspace#1}}}
\newcommand{\PS}[1]{\textcolor{blue}{[Puneet:]}{\textcolor{orange}{\xspace#1}}}
\newcommand{\ch}[1]{\textcolor{blue}{[Changhai:]}{\textcolor{orange}{\xspace#1}}}
\newcommand{\JY}[1]{\textcolor{blue}{[Jinsun:]}{\textcolor{orange}{\xspace#1}}}



% autoref section names
\renewcommand*\sectionautorefname{\Snospace}
\def\sectionautorefname{Sec.}
\def\subsectionautorefname{Sec.}
\def\subsubsectionautorefname{Sec.}
\def\figureautorefname{Fig.}
\def\algorithmautorefname{Alg.}


% Figure commands
\newcommand{\insertFigure}[5]{
    \begin{figure}[t]
      \centering
      \includegraphics[width=#3\linewidth]{figures/#1}
      \vspace{#4}
      \caption{\small #2}
      \label{fig:#1}
      \vspace{#5}
    \end{figure}
}

\newcommand{\insertFigureBoxed}[5]{%
  \begin{figure}[t]
    \centering
    \begin{tikzpicture}
      \node[draw, thick, red, inner sep=2mm] {%
        \includegraphics[width=#3\linewidth]{figures/#1}%
      };
    \end{tikzpicture}
    \vspace{#4}
    \caption{\small #2}
    \label{fig:#1}
    \vspace{#5}
  \end{figure}
}

\newcommand{\insertSubFigs}[9]{
  \begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.48\columnwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/#1}
      \caption{\centering #2}
      \label{fig:#3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\columnwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/#4}
      \caption{\centering #5}
      \label{fig:#6}
    \end{subfigure}
    \caption{\small #7}
    \label{fig:#8}
    \vspace{#9}
  \end{figure}
}

\newcommand{\insertFigureWide}[5]{
    \begin{figure*}[t]
      \centering
      \includegraphics[width=#3\linewidth]{figures/#1}
      \vspace{#4}
      \caption{\small #2}
      \label{fig:#1}
      \vspace{#5}
    \end{figure*}
}


\newcommand{\ArtifactBadges}{%
  \AddToShipoutPictureFG*{%
    \AtPageUpperLeft{%
      \hspace*{\dimexpr\paperwidth-4.8cm\relax}%
      \raisebox{-2cm}[0pt][0pt]{%
        \href{https://www.acm.org/publications/policies/artifact-review-and-badging-current}{%
          \includegraphics[width=1.35cm]{figures/artifacts-available-v1.1.pdf}%
        }\hspace{0.18cm}%
        \href{https://www.acm.org/publications/policies/artifact-review-and-badging-current}{%
          \includegraphics[width=1.35cm]{figures/artifacts-functional-v1.1.pdf}%
        }%
      }%
    }%
  }%
}

%%%% for tighter bullets
\newcommand{\squishlist}{
 \begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{3pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1.5em}
     \setlength{\labelwidth}{1em}
     \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
 \begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{0pt}
    \setlength{\topsep}{0pt}
    \setlength{\partopsep}{0pt}
    \setlength{\leftmargin}{2em}
    \setlength{\labelwidth}{1.5em}
    \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
  \end{list}  }





==> open-source-tools-old.tex <==
\section{Open-source Tools}
\label{sec:open-source-tools}
In this section, we introduce the open-source tools offered by the Chakra project, which are currently under active development. More tools can be added in the future.

\subsection{Execution Trace Linker}
\label{sec:chakra-trace-linker}

The \emph{Chakra Trace Linker} merges host-side (CPU) and device-side (GPU or NPU) execution traces into a unified representation. Collected independently, these traces are otherwise disjoint, limiting holistic reasoning about control flow and performance. The linker resolves this gap by establishing explicit cross-domain dependencies and producing a single dependency graph suitable for downstream performance analysis and simulation.

\paragraph{Why linking is necessary.}
Host traces collected through PyTorch’s Observer contain CPU activity and call stack information, while Kineto traces provide fine-grained timing information for kernels and operators. However, Kineto does not encode dependency information, and PyTorch Observer lacks detailed device timing. Neither source alone is sufficient to construct a comprehensive dependency graph. To address this gap, Chakra combines both sources: CPU information from the host trace and timing from Kineto. We also contributed a patch to PyTorch so that Observer and Kineto traces share common identifiers, allowing events to be matched across the two sources; this pull request has been merged upstream. Still, merging raw traces is not enough. In order to build a complete dependency graph suitable for analysis and simulation, we explicitly reconstruct multiple classes of dependencies—control, data, and synchronization—on top of the raw trace data. Concepts such as inter-stream and intra-stream dependencies, also discussed in systems like Lumos, are modeled in Chakra and integrated into the unified representation.

\paragraph{Control dependency.}
A control dependency indicates that the execution of one operation must follow another. 
For example, if function A calls function B, then B is control-dependent on A. 
Likewise, the return from B back to A also represents a dependency, since A cannot continue until B has completed. 
The linker reconstructs such causal ordering between host and device. 
This includes CPU function calls that launch kernels (CPU $\rightarrow$ GPU edges), 
returns or completion notifications from the device back to the host (GPU $\rightarrow$ CPU edges), 
and the ordering among host calls in the CPU call stack. 
These reconstructed links form the control-flow backbone of the unified trace 
and ensure that asynchronous operations are represented in the correct order.

\paragraph{Data dependency.}
Producer-consumer relationships are established by matching tensor identifiers and buffer handles across host and device. For example, when the CPU produces a tensor later consumed by a device kernel, or when a device kernel generates an output read by the host, the linker inserts explicit data edges. 
Similarly, two GPU kernels have producer-consumer relationship such as compute operation followed by communication operation (inter-stream dependency), compute operation followed by another compute operation  (intra-stream dependency), or hierarchical collective communication (inter-stream dependency) linker connects those with data edges. 
This guarantees that data movement and its dependent computation are represented consistently.

\paragraph{Synchronization dependency.}
The linker also inserts edges that capture ordering imposed by synchronization operations. This includes global synchronizations such as \texttt{cudaDeviceSynchronize()}, stream-specific calls like \texttt{cudaStreamSynchronize()}, and event-based coordination through \texttt{cudaEventRecord()} and \texttt{cudaStreamWaitEvent()}. Inspired by Holistic Trace Analysis (HTA)~\cite{hta_github}, these synchronization edges are treated as additional dependency constraints that extend the unified graph. 
By encoding them, the linker enables critical-path analysis and ensures that both explicit and implicit synchronization points are visible to downstream tools. 
% Chakra also explicitly distinguishes inter-stream and intra-stream dependencies, ensuring that ordering constraints within a stream as well as across streams are modeled consistently.

The implementation follows the design documented in the MLCommons Chakra project. The tool parses both CPU and device traces, resolves identifiers, and inserts control, data, and synchronization edges before emitting a unified dependency graph in the Chakra schema. This graph can then be passed to simulators or analyzed directly for bottleneck identification and scheduling studies.

\subsection{Execution Trace Converter}
\label{sec:execution-trace-converter}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/Dependency.pdf}
    \caption{Converted Trace example.}
    \label{fig:}
\end{figure}

\label{sec:pytorch-converter}

The Converter operates after the Linker and has two goals: (1) verify the dependencies produced by linking, and (2) emit a standardized Chakra ET graph.


\textbf{Dependency verification.}
The Converter checks the linked graph for structural soundness and removes artifacts that hinder analysis. It enforces acyclicity via standard topological validation, prunes false or redundant edges (e.g., edges contradicted by per-stream order or duplicating implied relations), reconciles inter- and intra-stream constraints into a consistent ordering, and validates process-group and domain consistency for communication nodes. All surviving edges are normalized into a single edge set with a \texttt{dep\_type} label (control/data/sync) and de-duplicated for determinism.

\textbf{Graph emission.}
Verified events are serialized into the Chakra schema as typed nodes (\texttt{COMP}, \texttt{MEM\_LOAD/MEM\_STORE}, \texttt{COMM\_SEND/RECV/COLL}) with optional timing hints (\texttt{start\_time\_micros}, \texttt{duration\_micros}) and extensible attributes (tensor sizes, ranks, group identifiers, tags, IO metadata). Edges are emitted as a cycle-free, canonical adjacency with stable ordering. The result is a single, standardized DAG that downstream tools (simulators, analyzers) can consume directly for scheduling studies, critical-path analysis, and performance modeling.

\textbf{Reference simulation.}
To demonstrate end-to-end usability, we provide a minimal simulation example that consumes the emitted Chakra ET graph and executes a policy-agnostic topological schedule (Kahn-style ready queue). The example illustrates how verified \texttt{dep\_type} edges and node attributes map to compute and communication events, serving as a concise template for integrating the Converter’s output with custom simulators.

% While various ML frameworks allow users to collect execution traces of ML models, they are often in different formats, hindering the exchange of traces between different organizations. The ET converter's role is to translate ETs from various schemas into the Chakra schema. Currently, the converter supports PyTorch and FlexFlow~\cite{jia2019beyond}, and considering that FlexFlow supports Keras, PyTorch, and ONNX, it can support most ML frameworks. TensorFlow support is planned for future work.

% The ET converter has prior knowledge of the input execution trace schema and can extract Chakra fields from the input file. For instance, PyTorch execution traces are in the JSON format, and the converter uses the JSON parser to read the execution traces. In PyTorch, computation nodes have the duration field if computation time is encoded after collecting traces, allowing computation nodes to be identified. Communication nodes in PyTorch are identified by the name of nodes, which is "record\_param\_comms". The communication type and size are determined by its child node, whose name starts with "nccl:". Unlike PyTorch traces, FlexFlow traces are in the graphviz format, and the FlexFlow codes needed to be slightly modified to identify node types and convey more metadata. Node types in FlexFlow are identified with the name field, and each node has corresponding metadata fields. One significant difference between FlexFlow and PyTorch is that collective communications in FlexFlow are broken down into multiple peer-to-peer data transfers. If the converter encounters uninterpretable nodes, they are classified as invalid nodes and ignored in other toolchains. It is important to note that in Chakra, each NPU generates a separate trace. Therefore, if an input file describes the behavior of all NPUs, the converter must split it into multiple pieces correctly.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.98\columnwidth]{figures/execution_graph_visualizer.pdf}
    \\
    \caption{Execution trace visualization example.}
    \label{fig:execution_trace_visualization_example}
    % alexnet with four GPUs generated by FlexFlow
\end{figure}

% \subsection{Execution Timeline Visualizer}
% \label{sec:execution-timeline-visualizer}
% The execution timeline visualizer presents task execution on each NPU in a timeline, taking a CSV file describing the task execution in a callback-based simulator. An example input format for the visualizer is presented in Snippet~\ref{snippet:timeline-visualizer-input-format}. The output timeline can be visualized with the trace event profiling tool in Chrome (chrome://tracing). \autoref{fig:execution_timeline_visualization_example} shows a screenshot of the visualization result, where tasks running on each NPU are presented as bars on the timeline, with their start and finish times. Tasks on an NPU are grouped as a process, and are classified into several sub-groups depending on the task type. In this example, two NPUs are shown, and memory access, computation, and communication have TID 1, 2, and 3, respectively. This tool allows researchers to easily identify bottlenecks in distributed ML tasks. For instance, in NPU 1, communication time is not overlapped with computation, unlike in NPU 2. Therefore, the task in NPU 1 can be optimized by overlapping communication with computation.

% \begin{figure}[!t]
% \begin{minipage}{\linewidth}
% \begin{lstlisting}[basicstyle=\footnotesize]
% issue,[gpu_id],[curr_cycle],[node_id],[node_name]
% callback,[gpu_id],[curr_cycle],[node_id],[node_name]
% issue,[gpu_id],[curr_cycle],[node_id],[node_name]
% issue,[gpu_id],[curr_cycle],[node_id],[node_name]
% callback,[gpu_id],[curr_cycle],[node_id],[node_name]
% callback,[gpu_id],[curr_cycle],[node_id],[node_name]
% ...
% \end{lstlisting}
% \vspace{-1em}
% \captionof{lstlisting}{Execution timeline visualizer input format.\ju{Remove?}}
% \label{snippet:timeline-visualizer-input-format}
% \end{minipage}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/execution_timeline_visualizer.png}
%     \\
%     \caption{Execution timeline visualization example.\ju{Alternate}}
%     \label{fig:execution_timeline_visualization_example}
% \end{figure}


\subsection{Dependency-Aware ET Feeder}
\label{sec:execution-trace-feeder}
% We offer a trace feeder library that is designed for simulators. One of the use cases for Chakra is simulating distributed ML systems for performance projection or what-if analysis. We anticipate that numerous companies and research institutions will actively share traces in the Chakra schema and use them with their simulators, whether open-source such as ASTRA-sim~\cite{rashidi2020astra, astrasim2} or SST~\cite{rodrigues2011structural}, or proprietary ones. The trace feeder library is implemented in C++, eliminating the need for users to repeatedly implement the parsing code. The trace feeder library significantly reduces users' engineering overhead. The public member functions of the trace feeder class are presented in Snippet~\ref{snippet:trace-feeder-class-definition}. With these functions, users can create a trace feeder instance and retrieve nodes or resolve dependencies.

The feeder ingests execution traces as a dependency graph and streams nodes to a simulator while strictly preserving the partial order defined by control and data edges. To bound memory usage, nodes are read in windows rather than loading the entire trace. When a node refers to a parent that has not yet appeared, it is placed into an unresolved set until the parent arrives. The feeder then elastically extends the window to resolve cross-boundary dependencies, ensuring correctness without preloading the full trace.

Each node maintains a count of unresolved predecessors. A node is ready once this count reaches zero and is inserted into a ready queue. The queue itself is policy-driven: nodes may be prioritized by measured start time, communication priority, or simply issued in FIFO order. Crucially, policies only arbitrate among ready nodes and therefore cannot violate dependency invariants. When a node completes, the feeder decrements the predecessor counts of its children, potentially unlocking new ready nodes. This process ensures that the emission order always respects the original dependency structure.

With this design, correctness is guaranteed by construction, while scheduling policy remains pluggable. The approach yields deterministic emission orders under a fixed policy, scales linearly with the size of the trace, and keeps memory usage proportional to the window size rather than the entire input. As a result, the feeder can support a variety of back ends—compute simulators while preserving the causal structure of the original execution trace.

% \subsection{Test Case Generator}

% While execution traces are expressive and can effectively encode real-world ML traces, their limited readability poses challenges for implementing ET-based tools. The test case generator allows users to define arbitrary execution traces that can subsequently be used to generate test cases. Additionally, the test case generator allows manual modeling of ML models. The test trace generator offers an array of C++ classes for composing Chakra execution traces. Snippet~\ref{snippet:synthetic-trace-generator-example} demonstrates how an execution trace can be defined within the tool. As illustrated in the code snippet, users can create a new trace and designate the dependencies between nodes. We also offer several default trace examples, encompassing data parallel, model parallel, and pipeline parallel instances for a synthetic ML model.

\subsection{Execution Trace Visualizer}
\label{sec:execution-trace-visualizer}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/cdf_node_duration.png}
    \caption{Cumulative Distribution Function of Node Durations. \ju{Could be more flatten and redable.}}
    \label{fig:cdf}
\end{figure}

The execution trace visualizer is designed to visualize execution traces in the Chakra schema.
An example of a visualization from the execution trace visualizer is presented in \autoref{fig:execution_trace_visualization_example}.
The visualizer's input file should conform to the Chakra schema, and it can output files in either the graphviz or PDF format. 
The visualizer is a helpful tool for researchers to understand the structure of execution traces. Moreover, it can be used for debugging simulators or emulators that take Chakra execution traces. By default, the visualizer encodes the names of tasks and dependencies between tasks. 
Users can easily modify the visualizer to encode additional metadata such as compute time and communication size. 
\ju{
Figure~\ref{fig:cdf} demonstrates the distribution of compute node durations across different time scales.
}
% \begin{figure}[!t]
% \begin{minipage}{\linewidth}
% \begin{lstlisting}[basicstyle=\footnotesize]
% et = new DependencyGraph(getFilename(..., npu_id));

% node1 = et->addNode(ChakraProtoMsg::COMP_NODE);
% node1->set_name("COMP_NODE");
% node1->set_simulated_run_time(5);

% node2 = et->addNode(ChakraProtoMsg::COMP_NODE);
% node2->set_name("COMP_NODE");
% node2->set_simulated_run_time(5);

% et->assignDep(node1, node2);
% \end{lstlisting}
% \captionof{lstlisting}{Test case generator codes.}
% \label{snippet:synthetic-trace-generator-example}
% \end{minipage}
% \end{figure}

% \begin{figure}[!t]
% \begin{minipage}{\linewidth}
% \begin{lstlisting}[basicstyle=\footnotesize]
% void addNode(std::shared_ptr<EGFeederNode> node);
% void removeNode(uint64_t node_id);
% bool hasNodesToIssue();
% std::shared_ptr<EGFeederNode> getNextIssuableNode();
% void pushBackIssuableNode(uint64_t node_id);
% std::shared_ptr<EGFeederNode> lookupNode(uint64_t node_id);
% void freeChildrenNodes(uint64_t node_id);
% \end{lstlisting}
% \captionof{lstlisting}{Trace feeder class public member functions.}
% \label{snippet:trace-feeder-class-definition}
% \end{minipage}
% \end{figure}


==> overview-old.tex <==
\section{Chakra Overview}
\label{sec:chakra}
In this section, we overview Chakra, a performance modeling framework for distributed ML workloads. Comprising various concepts and tools, Chakra enables users to estimate the execution time and resource usage of a distributed ML task for a given system configuration. \autoref{fig:Chakra_infrastructure_overview} illustrates the key components of the Chakra infrastructure, with execution traces (ETs) serving as the central element. These ETs facilitate the exchange of ML execution traces without revealing model specifics. Generated by ML frameworks, ETs are converted to a common format, \Chakraet, which are subsequently fed into simulators to estimate the performance of ML workloads. In this section, we provide an overview of the Chakra project and its main components.

\subsection{Motivation}
\label{sec:motivation}
The importance of HW-SW codesign in designing distributed ML systems is well-known. Despite its importance, the necessary infrastructure for effective implementation remains insufficient. Three primary challenges hinder progress in this area. Firstly, the absence of a unified schema for exchanging execution traces of ML models poses a significant obstacle. Although numerous ML frameworks and languages exist, their primary focus has been on representing and optimizing ML models, with performance modeling receiving less attention. Consequently, no standard schema for encoding execution information has been developed. Secondly, the lack of toolchains for performance modeling is another challenge. Comprehensive toolchains are crucial for identifying bottlenecks and debugging issues efficiently. Lastly, sharing traces across organizations and researchers remains difficult due to proprietary constraints. Traces obtained from real executions and, when needed, synthetic traces that preserve key execution characteristics enable safe exchange and support performance projection for systems with varying system sizes and interconnect configurations.

\subsection{Schema}

In Chakra, execution traces are in the Chakra schema, which is defined as a common format for exchanging execution traces for performance modeling purposes. The need for a standardized schema arises as ML frameworks often provide methods to collect execution traces of ML models, but these traces are presented in varying formats, which obstructs the exchange of information between different organizations. To address this issue, the Chakra schema is designed based on the requirements of various organizations, including universities and companies. Moreover, the schema facilitates the collection of traces at different stages, such as pre-execution and post-execution, allowing for the gathering of traces that are either specific to a particular system design or not.

\begin{figure}[t]
    \centering
    \includegraphics[width=.98\linewidth]{figures/Chakra_overview_2.pdf}
    \caption{Chakra infrastructure overview.}
    \label{fig:Chakra_infrastructure_overview}
\end{figure}

\subsection{Chakra ET Collection and Synthesis}
\label{sec:et-sources}
% Execution traces can be collected from real-world ML frameworks or synthetic trace generators, each with its own pros and cons. ML frameworks offer the most straightforward method for collecting execution traces, as they run ML models directly. We extended PyTorch to support trace collection with the Execution Graph Observer~\cite{pytorch_eg_observer}, which does not require intrusive modifications to ML models. Simply enabling the Execution Graph Observer before running a model yields traces that closely reflect real-world execution.
% In addition, Chakra is officially supported as an option in NVIDIA NeMo, which allows users to enable Chakra trace generation within the NeMo workflow.

Execution traces can be collected from real-world ML frameworks or from synthetic generators, each with its own tradeoffs. ML frameworks provide a direct path because models run as is. We extended PyTorch with the Execution Graph Observer~\cite{pytorch_eg_observer}, which we refer to as the CPU trace, and Kineto~\cite{pytorch_kineto}, which we refer to as the device trace. These tools do not require intrusive modifications, and once enabled, the collected traces reflect different aspects of execution outcomes. In addition, Chakra is officially supported as an option in NVIDIA NeMo~\cite{nvidia_nemo}, which allows users to enable Chakra trace generation within the NeMo workflow.

This approach is faithful but tied to the concrete system. To decouple these factors when needed, Chakra traces can also be generated synthetically, preserving key execution characteristics for projection and controlled sharing.

Existing work has also explored synthetic or pre-execution approaches for trace generation. For example, STAGE constructs symbolic tensor graphs based on system analysis, enabling scalable synthesis of LLM benchmarks without relying on a specific runtime environment~\cite{stage}. In another approach, LayerDAG leverages generative AI models to synthesize execution traces in order to obfuscate intellectual property while retaining representative performance characteristics~\cite{li2024layerdag}. These approaches highlight complementary motivations: STAGE emphasizes scalability and coverage of large models in a pre-execution setting, while LayerDAG emphasizes protecting intellectual property from trace release. Chakra’s design accommodates both real post-execution traces and synthetic pre-execution traces, making it a bridge between faithful replay and scalable, privacy-preserving synthesis.

% \ju{This overlaps with STG a lot. Should shrink..}
% Synthetic trace generators can overcome these limitations. In our study, we designed a generative ML model trained with production traces to capture the characteristics of ML traces, such as the relationships between nodes in a trace and their fields. This model can be used to simulate traces of various ML models by varying the number of NPUs. A key advantage of the generative ML model is its ability to obfuscate traces, which is critical for sharing ML traces while protecting intellectual property. Obfuscation is a significant concern when sharing ML traces, and the generative ML model can address this issue by conveying the essential characteristics of the trace while maintaining privacy.

\subsection{Open-source Tools}
Chakra offers a range of open-source tools to help users modify and better understand the execution traces. These tools include the execution trace converter, execution trace visualizer, timeline visualizer, test case generator, and execution trace feeder, all of which are currently available on our GitHub repository\footnote{https://github.com/mlcommons/chakra} and under active development. The execution trace converter is responsible for converting execution traces in various schemas to the Chakra schema. The execution trace visualizer allows users to visualize the dependencies between nodes in a trace. Meanwhile, the timeline visualizer provides a visualization of the execution of nodes when a trace is simulated in a simulator. The test case generator lets users generate arbitrary execution traces by offering libraries to describe traces. The execution trace feeder is a library that other simulators can use to parse traces and feed them into the simulator. Further details will be presented in \autoref{sec:open-source-tools}.

\subsection{Use Cases}
\label{sec:use-cases}

Chakra enables multiple use cases by providing a unified schema for execution traces that can be consumed across frameworks and toolchains. Three key applications are:

\begin{itemize}
  \item \textbf{Model performance analysis.} Chakra traces capture detailed compute and communication behavior, allowing developers to identify bottlenecks, compare parallelization strategies, and guide kernel and model level optimizations without exposing model or dataset details.
  \item \textbf{Infrastructure and hardware evaluation.} The same traces can drive simulators and replayers to estimate performance under alternative GPU/NPU counts, network topologies, or system configurations. This supports hardware software codesign and investment planning while letting organizations use their own internal tools as long as they adopt the common format.
  \item \textbf{Benchmarking and trace sharing.} A standardized schema makes it possible to exchange traces across teams and organizations, enabling fair benchmarking, collaborative analysis, and broader community engagement without revealing proprietary models or datasets.
\end{itemize}


% \subsection{Use Cases} 
% \ju{Explain with two bullet. Model performance / Infra+HW performance.}
% Chakra serves a variety of purposes, including HW-SW co-design, benchmarking, and performance projection. The proposed Chakra schema serves as a unified format for exchanging execution traces, significantly simplifying the process of sharing these traces. Additionally, the generative AI model enables users to produce representative traces based on existing ones. As a result, NPUs or training systems can be optimized using these traces. Furthermore, Chakra can be employed for performance projection, allowing users to estimate the potential performance improvements resulting from investments by modeling systems with varying compute engines or network topologies. A key advantage of Chakra is that it allows companies to use their own internal simulators or toolchains, provided they follow the common format.

==> overview.tex <==




==> reviews/CAL.tex <==
Dear Dr. Heo:

Manuscript CAL-2022-09-0126 entitled "MLSimPerf: Enabling Pre-silicon Co-design for ML Systems" which you submitted to the IEEE Computer Architecture Letters, has been reviewed.  The comments of the reviewer(s) are included at the bottom of this letter.

The reviewers feel that your submission is promising, but have indicated significant concerns.  Before they can further evaluate it, they have requested some major revisions. Therefore, we invite you to respond to the editor's and reviewer(s)' comments and then revise and resubmit your manuscript. The resubmission will be given a new manuscript ID but will be linked to the previous version and will be sent back to the reviewers for their evaluation.  

In order to preserve the immediacy that is part of Computer Architecture Letters' mission, the resubmission should be completed within six weeks.  Furthermore, please note that ONLY ONE REVISE & RESUBMIT IS ALLOWED. If the resubmission does not sufficiently address the reviewers concerns, we must decline to publish the work.

To revise your manuscript, log into https://mc.manuscriptcentral.com/cal and enter your Author Center, where you will find your manuscript title listed under "Manuscripts with Decisions."  Under "Actions," click on "Create a Resubmission."  

Please be sure to include a separate response file indicating how you have addressed each of the editor's and reviewer(s)' comments. In order to expedite the processing of the revised manuscript, please be as specific as possible in your responses.

Once the revised manuscript is prepared, you can upload it and submit it through your Author Center. IMPORTANT:  Please submit camera-ready copy.  You must use the Computer Architecture Letters template, available at https://www.computer.org/publications/author-resources/peer-review/journals#templates.


Once again, thank you for submitting your manuscript to the IEEE Computer Architecture Letters and we look forward to receiving your resubmission.


Sincerely,

IEEE Computer Architecture Letters Editorial Office


---


Associate Editor
Comments to the Author:
Dear Authors,

Please address reviewer's concerns thoroughly. In particular strengthen the evaluation section by adding more results using proposed simulator and add more details on various aspects of the paper such as, obfuscation and reverse engineering.


Reviewer(s)' Comments to Author:

Reviewer: 1

Recommendation: Minor Revision

Comments:
(There are no comments. Please check to see if comments were included as a file attachment with this e-mail or as an attachment in your Author Center.)

Additional Questions:
1. Confidence in your review: High

2. What is the important insight or idea that this paper contributes?: The paper proposes MLSimPerf, which is an infrastructure that enables the benchmarking of ML models represented by execution graphs. The execution graphs encode compute and communication operator dimensions and dependencies. As the execution graphs do not reveal any model or dataset details, they can be shared between SW and HW vendors/academia without exposing proprietary information. This allows HW vendors to better optimize their design for the ML models and to provide feedback to the SW vendors allowing the optimization of compute and network configurations.

3. What is the potential impact of this paper?: It is an incremental improvement on the state of the art execution graphs converting them into a common format. The contribution is the obfuscation of the execution graph details.

However, I am not sure that the execution graph format as proposed in the publication is generally applicable to test all machine learning architectures. Some architectures like for example Cerebras/Graphcore use compilers that leverage detailed model information - which is subject to the obfuscation - to optimize scheduling / mapping / communication between their compute units.

6. Other comments for the authors: It is unclear how the memory accesses can be accurately modelled based on the number of accesses only, as the cache miss rate recorded yields little information to the simulator and the interconnect BW is a frequent bottleneck in state of the art system designs. If the memory addresses accessed and the resulting pattern is to be made obscure, can the model be improved with probability distributions for example average accessed address distances and sharing patterns?

Can the approach be applied on machine learning architectures that use compilers to optimize the model execution? What are the limitations of the proposed execution graph approach - especially considering obfuscation?

5. What revisions do you suggest for the paper?: I think the numbers were meant to be 0 and 1 for the NPUs in the following sentence:
"In NPU 1, communication time is exposed unlike in NPU 2."

The validation section should be improved.
In addition to running only two collective communication primitives actual benchmarks should be run.
It would be great if the Astra-sim-v1 simulator could be included in the future system simulation section to improve the validation and verifying the MLSimPerf execution graph method accuracy. The validation section as it is, is not detailed enough to fully convince me of the precision of the approach. While the benefits of the approach are clear and intuitive to me and I like the future system simulation design space exploration, I would have preferred a more thorough validation.

The results presented in figure 5 do not convey much information as it is only shown that the latency scales for both simulators approximately linearly with an increase in the message size for the selected configuration. As the communication patterns are quite uniform the results presented can be expected.

4. Is the manuscript technically sound?  Please explain your answer in
the "revisions" or "comments for the authors" sections below.: Yes


Reviewer: 2

Recommendation: Minor Revision

Comments:
(There are no comments. Please check to see if comments were included as a file attachment with this e-mail or as an attachment in your Author Center.)

Additional Questions:
1. Confidence in your review: Medium

2. What is the important insight or idea that this paper contributes?: The core of MLSimPerf is to convert the ML models into execution graphs. Then, the MLSimPerf framework utilizes an improved version of Astra-sim to model the performance based on these execution graphs

3. What is the potential impact of this paper?: - The tool enables HW-SW co-design while protecting the IPs, which will be very useful for future design.

6. Other comments for the authors: This paper presents MLSimPerf, which is a simulation framework for HW-SW co-design for ML applications. The core of MLSimPerf is to convert the ML models into execution graphs. MLSimPerf's execution graph can take a different type depending on the core operation of each node (compute/memory/communication/special). Then, the MLSimPerf framework utilizes an improved version of Astra-sim to model the performance based on these execution graphs. Finally, the MLSimPerf framework includes a graph converter that allows different ML models to work with the MLSimPerf framework. The key result of the paper includes validation for the communication node as well as design exploration using MLSimPerf.

Pros:
- The tool enables HW-SW co-design while protecting the IPs, which will be very useful for future design.
- EG seems framework agnostic.

Cons:
- The contribution over Astra-sim seems incremental.
- Limited validation results. Only communication nodes are validated against an older version of Astra-sim.


Overall, I like the direction of the paper and I believe that MLSimPerf will become a good tool for HW-SW co-design for ML applications. The types of nodes available should be able to cover major ML models currently available. I appreciate the presented data that includes the validation for the communication node. However, there are also some issues with the current version that should be addressed if this work is to be extended into a conference submission.

First, I think the paper is somewhat incremental considering what Astra-sim can currently do. Specifically, this work introduces a method to allow the performance model to take into account different phases of ML programs through the execution graph. Because most ML frameworks likely will have their own internal execution graph, the main contribution of this work is on how to ensure that the execution graph from each framework is compatible with each other through the graph converter. However, it is unclear from the paper how the execution graph converter really works.

Second, the validation results only include the communication node. While the communication node is likely more challenging to model, presenting the comparison between Astra-sim v2 and Astra-sim v1 as validation results do not seem like a good methodology. The paper will benefit from more validation data that spans more node types as well as more ML models on real hardware.

5. What revisions do you suggest for the paper?: - Please try to expand Section 2.3 with somewhat more detail on how this can be done.
- Please provide additional validation results vs. real ML workload if possible

4. Is the manuscript technically sound?  Please explain your answer in
the "revisions" or "comments for the authors" sections below.: Yes


Reviewer: 3

Recommendation: Minor Revision

Comments:
(There are no comments. Please check to see if comments were included as a file attachment with this e-mail or as an attachment in your Author Center.)

Additional Questions:
1. Confidence in your review: Medium

2. What is the important insight or idea that this paper contributes?: The paper proposes a novel execution graph format, MLSimPerf_EG, to be used in performance modeling for HW/SW co-design. The EG can be automatically extracted from existing ML frameworks, does include dependency&trace information, and be used to estimate the real traces even when the model is obfuscated.

3. What is the potential impact of this paper?: The proposed approach has the potential to let ML HW vendors estimate performance without needing the actual model and determine bottlenecks to feed back to the model designer.

6. Other comments for the authors: The overall idea is novel and widespread adoption would enable efficient HW/SW co-design. I believe MLSimPerf_EG can significantly accelerate determining optimal architectural hyperparameters. I have the following questions:

1. How do you comment on ONNX's use as a tool for performance modeling? Would it be feasible in the longer term to have a translation layer that transforms such a higher layer model to EG traces?

2. What is the maximum degree of detail the computation nodes can be modeled without compromising model confidentiality? As far as I understand, if an ML HW vendor tries to explore the compute design space, i.e., play with superscalar ISAs or different arithmetic representation formats, MLSimPerf_EG has little to offer -- for the compute primitives, such metadata should be separately obtained. I believe a fused approach that includes more design parameters for the computation primitives would be extremely helpful since compute optimization is on the critical path for many models.

5. What revisions do you suggest for the paper?: -Exposed communication time is mentioned in 2.4 but defined in 3.1, would be good to have it defined earlier to make the paper easier to read.
-If there's enough space, would be good to have pointers for my questions in the comments to the authors section.

4. Is the manuscript technically sound?  Please explain your answer in
the "revisions" or "comments for the authors" sections below.: Yes


Reviewer: 4

Recommendation: Minor Revision

Comments:
(There are no comments. Please check to see if comments were included as a file attachment with this e-mail or as an attachment in your Author Center.)

Additional Questions:
1. Confidence in your review: Medium

2. What is the important insight or idea that this paper contributes?: This paper presents MLSimPerf, a ML benchmark infrastructure that allows performance evaluation of proprietary models without disclosing the model parameters (IP). This is made possible through the design of a common intermediate abstraction in the form of an Execution Graph (EG).

3. What is the potential impact of this paper?: The idea proposed in this work has a few potential merits -

i) It allows organizations to transparently share performance benchmarks for their models while keeping thier IP private, facilitating HW/SW co-design.

ii) It attempts to maintain a common standard for workload execution traces that can potentially be made compatible with any workload system simulator.

iii) As an initial starting point, the authors provide adapters for converting EGs from PyTorch, a popular open-source ML framework. They also update ASTRA-sim, an existing system sim to be compatible with MLSimPerf EGs. Visualization tools are also provided to graph MLSimPerf EGs.

6. Other comments for the authors: A few concerns about this work -

i) Designing adapters to support individual ML frameworks is not trivial. Some frameworks may generate EGs with metadata that may not directly translate to the MLSimPerf format. Can there be information loss in translating such EGs?

ii) How can the accuracy of a converted EG be verified? Can there be a validation tool that formally verifies that the original framework EG and the MLSimPerf EG are functionally the same? This is crucial if other organizations are to design systems based on the simulation results from the MLSimPerf EG.

iii) How difficult is it to reconstruct the model, given a set of EGs for a bunch of workloads? The authors mention plans for implementing an obfuscation tool to mitigate RE attempts. How does 'minor changes' to the EG for obfuscation purposes affect the actual execution trace data? Won't this fudge the accuracy of the benchmark results?

iv) Although having a common standard is good for the community, I don't see why the organizations cannot share the EGs from the existing ML frameworks directly? HW and system developers may be using simulators that are already compatible with the popular ML frameworks. What is the incentive to update their proprietary simulators to support yet another format instead of ingesting EGs from frameworks they already support?

5. What revisions do you suggest for the paper?: The primary pitch for the paper was to develop an ML infrastructure to protect model IP. However, this paper lacks details about how this can be achieved. Some details about how an EG mitigates reverse engineering model parameters would strengthen the paper. Also, further discussion about how the authors plan on implementing the obfuscation layer would be helpful.

4. Is the manuscript technically sound?  Please explain your answer in
the "revisions" or "comments for the authors" sections below.: Yes


Reviewer: 5

Recommendation: Revise & Resubmit (paper requires more than a minor revision)

Comments:
(There are no comments. Please check to see if comments were included as a file attachment with this e-mail or as an attachment in your Author Center.)

Additional Questions:
1. Confidence in your review: Medium

2. What is the important insight or idea that this paper contributes?: This paper presents a simulation methodology to enable simulation of proprietary ML models through the use of a novel execution graph abstraction without exposing model details.

3. What is the potential impact of this paper?: + Enable execution graph traces of industry / closed-source ML models.
+ Standard simulation methodology infrastructure for a variety of ML frameworks.

6. Other comments for the authors: This paper presents an execution graph abstraction to enable performance modeling of ML models without exposing model architecture details. Given the 4 page limit of CAL, the paper does a fairly good job at discussing the components of the simulation infrastructure and getting the main points across.

My main critique of this work is that the evaluation section can be more focused on evaluating the contribution of this paper (novel EG abstraction). As of now, the evaluation appears to be a generic demonstration of ASTRA-sim in general. Many of the experiments could have been carried out with ASTRA-sim-v1. The paper would be made stronger if the evaluation scenarios better highlight the possibilities that ASTRA-sim-v2 can provide that ASTRA-sim-v1 couldn't. If the existing experiments already do this, then it is not clear to me and motivating the evaluation with through this lens would be more effective.

5. What revisions do you suggest for the paper?: Please address the following:

* How are nodes determined to be unnecessary for performance modeling?

* How are execution graphs partitioned across NPU?

* The performance model validation presents a collective communication primitive. The change for ASTRA-sim-v2 lies in the workload layer. I'm not seeing how this test case validates changes made to the workload layer. It appears this validation experiment tests the system layer and lower, but misses the workload layer where modifications were made.

* In Page 3: "Performance is defined as the reverse of execution cycles" Did you mean "inverse" instead of "reverse"?

4. Is the manuscript technically sound?  Please explain your answer in
the "revisions" or "comments for the authors" sections below.: Yes

==> reviews/MLBench.tex <==
Dear Authors,

Thank you for submitting to MLBench'23.  We are pleased to inform you that your submission has been selected for inclusion in our workshop.

The next deadline is to send us a camera-ready version of your paper by May 19.

Please remember that the workshop is being held in-person, so don't forget to make your travel arrangements.

Tom St. John, Murali Emani, Wenqian Dong

SUBMISSION: 5
TITLE: Chakra: Advancing Performance Benchmarking and Co-design using Standardized Execution Traces


----------------------- REVIEW 1 ---------------------
SUBMISSION: 5
TITLE: Chakra: Advancing Performance Benchmarking and Co-design using Standardized Execution Traces
AUTHORS: Srinivas Sridharan, Taekyung Heo, Louis Feng, Zhaodong Wang, Matt Bergeron, Wenyin Fu, Shengbao Zheng, Brian Coutinho, Saeed Rashidi, Changhai Man and Tushar Krishna

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
Thank you for submitting this work to MLBench23! I enjoyed reading this paper and I can't wait to use the tools.

The idea to take existing execution traces and convert them into a universal format, and then use generative models to create traces that are similar but do not give away companies' IPs makes a lot of sense.

Overall, the paper is clear, well motivated, and it presents a neat idea.

I encourage the authors to include a link to the Chakra repository, as right now there are several online tools called Chakra, making this work difficult to find.

Overall, I do not have many suggestions for improvement. The one idea I would have liked to see developed more was the technical issues (if any) that authors faced when converting PyTorch/FlexFlow traces in the Chakra format, and what the authors estimate would be the challenges of doing the same for Tensorflow.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 5
TITLE: Chakra: Advancing Performance Benchmarking and Co-design using Standardized Execution Traces
AUTHORS: Srinivas Sridharan, Taekyung Heo, Louis Feng, Zhaodong Wang, Matt Bergeron, Wenyin Fu, Shengbao Zheng, Brian Coutinho, Saeed Rashidi, Changhai Man and Tushar Krishna

----------- Overall evaluation -----------
SCORE: 1 (weak accept)
----- TEXT:
In this work, the authors have proposed Chakra, a system that facilitates performance-modeling and co-design of ML HW+SW based on an execution trace schema.

The work is motivated by difficulties in collecting, sharing, and using execution traces due to the lack of a standard schema. The authors define the schema, present a generative model approach for synthesizing traces, and nicely provide open source tools for using these traces. The design requirements of the schema were informed by surveying various teams and organizations.

The generative model aspect to Chakra is described as essential to solve certain problems, but the model is not fully explained, nor are there any results that evaluate its quality.

It would be nice to show more actual examples of traces, and show how different stages of execution are represented. It would help with understanding and make the design seem less abstract. Also, I think a little more explanation is needed on specific differences between execution graphs and traces.



----------------------- REVIEW 3 ---------------------
SUBMISSION: 5
TITLE: Chakra: Advancing Performance Benchmarking and Co-design using Standardized Execution Traces
AUTHORS: Srinivas Sridharan, Taekyung Heo, Louis Feng, Zhaodong Wang, Matt Bergeron, Wenyin Fu, Shengbao Zheng, Brian Coutinho, Saeed Rashidi, Changhai Man and Tushar Krishna

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
This paper introduces Chakra which is a framework for performance modeling with the help of Execution Trace. The research direction is promising with well-worded motivation and introduction. The paper organization is somewhat confusing at first glance due to repetitiveness and cross-referencing inside the paper.

Here are some minor comments.
* The explanation can be improved regarding how exactly the synthetic trace generators help to decouple from hardware.

* The paper mentions chakra approach is good for hardware-software co-design. Additional explanation and experimental case study can be helpful to solidify this claim.

* There is a discussion regarding generative AI models in Section 4. However, more details on how exactly they are used in the context of current work are sparse. Detailed case study and explanation in the text can be helpful.


* Performance projection is discussed several times in the work. However,  experimental evaluation lacks a comparison between projected performance and actual measured performance for an application.

* No reference to Figure 2 in a text (perhaps in section 4)
* No reference to Figure 6 in a text (perhaps in section 6.2.4)


==> schema-old.tex <==
\section{Chakra Schema}
\label{sec:schema}

The Chakra schema provides a standardized representation of execution traces for machine learning workloads. The goal is to capture execution in a form that is portable across frameworks and extensible for diverse use cases, while remaining compact and easy to consume by analysis tools and simulators.

\subsection{Design Requirements}
\label{sec:chakra-schema-design-requirements}

Machine learning tasks are naturally expressed as graphs, with frameworks such as TensorFlow and PyTorch constructing internal computational graphs~\cite{computational_graphs}. In this work, we generalize this idea to \textit{execution traces} (ETs), graphs that record not only model structure but also execution details such as memory accesses, compute operations, communication, and parallelization strategies. Although ETs are a powerful abstraction, their structure and metadata differ across frameworks, limiting reuse.

The Chakra schema was designed through discussions with both academic and industrial teams to meet several requirements. First, the schema must be minimal yet extensible: only essential fields should be mandatory, but attributes should allow customization without modifying the core definition. Second, the schema must be expressive for performance modeling: it should capture computation, memory, communication, and their dependencies. Third, the schema must be portable across levels of abstraction: traces should be usable for both real system replay and projection to future system configurations.

The schema can capture traces at different stages of execution. 
At the pre-execution stage, traces are not tied to a specific hardware 
configuration, which makes them useful for performance projection. 
At the post-execution stage, traces reflect the actual system behavior 
including optimizations and parallelization strategies, which is 
valuable for diagnosing bottlenecks. Chakra accommodates both levels 
without modifying the schema.

\subsection{Schema}
\label{sec:chakra-schema-detail}

The schema represents execution as a directed acyclic graph (DAG) where nodes denote operations and edges encode data and control dependencies. Instead of fixing a large set of operators, Chakra defines a small set of node categories together with an attribute mechanism for extension. This ensures portability while allowing new operators or system-specific annotations to be added without breaking compatibility. Communication is modeled explicitly as a node type alongside computation and memory, enabling consistent representation of parallelization strategies and system-level effects. By unifying these elements, the schema supports performance analysis and hardware–software codesign without exposing proprietary model or dataset details.

\begin{table}[t!]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|}
    \hline
    \textbf{Field Name} & \textbf{Data Type} & \textbf{Description} \\ \hline
    id                  & uint64             & Unique node identifier \\ \hline
    name                & string             & Human-readable name \\ \hline
    type                & enum(NodeType)     & Node category (compute, memory, communication) \\ \hline
    ctrl\_deps          & repeated uint64    & Control dependencies \\ \hline
    data\_deps          & repeated uint64    & Data dependencies \\ \hline
    start\_time\_micros & uint64             & Optional start time \\ \hline
    duration\_micros    & uint64             & Optional duration \\ \hline
    inputs/outputs      & IOInfo             & Values, shapes, types \\ \hline
    attr                & repeated AttributeProto & Extensible metadata \\ \hline
    \end{tabular}
    }
    \caption{Chakra node schema.}
    \label{tab:chakra-node-schema}
\end{table}

Each node (\autoref{tab:chakra-node-schema}) contains a unique identifier, a name, and a type that specifies whether it represents computation, memory, or communication. Control and data dependencies define the partial order, allowing the feeder to reconstruct execution. Optional timing fields capture start and duration hints. 
Inputs and outputs are described through \texttt{IOInfo}, which records identifiers, shapes, and data types of tensors. This allows each node to be linked consistently to the tensor schema without requiring a separate table in the main text.

\begin{table}[t!]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|}
    \hline
    \textbf{Field Name} & \textbf{Data Type} \\ \hline
    type & enum(CommType): AllReduce, AllGather, ReduceScatter\\
     & Broadcast, Point-to-Point, All2All, Barrier \\ \hline    group       & uint64 \\ \hline
    tag         & string \\ \hline
    tensor\_ids & repeated uint64 \\ \hline
    \end{tabular}
    }
    \caption{Chakra communication schema.}
    \label{tab:chakra-comm-schema}
\end{table}

Communication nodes describe collective and point-to-point operations. 
The \texttt{type} field enumerates supported communication primitives. 
The \texttt{group} field specifies the set of ranks involved in the operation, 
and the optional \texttt{tag} helps distinguish concurrent operations. 
The \texttt{tensor\_ids} field links the communication to tensor objects 
defined in the tensor schema.

Chakra maintains per-device traces, which simplifies collection and replay. 
To represent distributed execution across devices, communication nodes 
include a group identifier that specifies the ranks involved in a collective. 
This mechanism, similar to process groups in PyTorch, allows complex forms 
of parallelism such as tensor, pipeline, data, and expert parallelism to be 
expressed consistently within the schema.

\begin{table}[t!]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|}
    \hline
    \textbf{Field Name} & \textbf{Data Type} \\ \hline
    id      & uint64 \\ \hline
    storage\_id & uint64 \\ \hline
    storage\_offset & uint64 \\ \hline
    shape   & repeated int64 \\ \hline
    stride  & repeated int64 \\ \hline
    dtype   & enum(DataType): fp16, bf16, fp32, int8, etc. \\ \hline
    size\_bytes & uint64 \\ \hline
    \end{tabular}
    }
    \caption{Chakra tensor schema.}
    \label{tab:chakra-tensor-schema}
\end{table}

\begin{table}[t!]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|}
    \hline
    \textbf{Field Name} & \textbf{Data Type} \\ \hline
    id      & uint64 \\ \hline
    size\_bytes & uint64 \\ \hline
    device  & string \\ \hline
    \end{tabular}
    }
    \caption{Chakra tensor storage schema.}
    \label{tab:chakra-tensor-storage-schema}
\end{table}

Tensor descriptors capture the structure and placement of data. 
Each tensor has a unique identifier, shape, and data type, with 
the \texttt{size\_bytes} field recording its storage footprint. The \texttt{storage\_id} field records the physical memory on which this tensor is allocated with \texttt{storage\_offset} to define the offset in that physical memory. Splitting tensor and its storage makes it possible to support tensor alias, for example, two tensors share the same storage but with different shapes. These descriptors allow compute and communication nodes to be linked consistently through tensor references. Tensor storage node represents a unique physical memory, it has a unique id, the memory size, and the device the storage resides.
This design satisfies the requirements in \autoref{sec:chakra-schema-design-requirements}. It is \emph{minimal yet extensible}, containing only core fields while supporting rich metadata through attributes. It is \emph{expressive}, capturing computation, memory, and collective or point-to-point communication. Finally, it is \emph{portable}, accommodating traces collected at different abstraction levels and consumable by diverse simulators.


% This section provides a detailed description of the Chakra schema. In this section, we present the goal of the schema and its design. Additionally, we discuss the important design choices made during the development of the Chakra schema.

% \subsection{Design Requirements}
% \label{sec:chakra-schema-design-requirements}
% ML tasks are often presented as graphs, with frameworks such as TensorFlow and PyTorch constructing computational graphs internally to represent model execution~\cite{computational_graphs}. In this study, we introduce \textit{an execution trace} (ET) as a graph that captures the execution details of an ML task. An ET is a trace of ML execution that includes details such as memory accesses, computational load, network communication, and parallelization strategies. While ETs are a useful way to represent an ML task, the structures and metadata of generated ETs may differ depending on the ML framework used. To ensure that the Chakra framework can be used across different ML frameworks, we propose a standard ET schema for performance modeling called Chakra execution trace (\Chakraet).

% The Chakra schema was designed to meet the diverse requirements of various teams and organizations. To achieve this goal, we had meetings with many universities and companies to gather input from different teams. We present the requirements that were incorporated into the schema. The first requirement is that the schema should be minimal yet extensible. This is a common requirement across all organizations because they do not want to use up resources on non-used fields, but they also want to extend the schema for their specific purposes. The second requirement is that the schema should be able to model various aspects of ML execution from a performance modeling perspective. While there are many languages and representations designed for presenting ML models, there is no common schema for modeling the performance of ML execution. Therefore, performance modeling is a critical aspect of schema design. The schema should be able to model memory access, computation, and network communication. Additionally, the trace should have dependencies between nodes because many operations have dependencies. The third requirement is that the schema should be able to present execution traces at different stages of execution. If the resulting trace is too tightly coupled to the real system execution, it cannot be used for performance projection or estimation. Therefore, the schema should be able to present execution traces at any level of ML execution.

% \subsection{Schema}
% \label{sec:chakra-schema-detail}

% The Chakra schema is designed to provide a common representation of execution traces that can be shared across frameworks and systems. Its central idea is to view execution as a directed graph where nodes represent operations and edges represent data and control dependencies. Instead of prescribing a fixed set of operators, the schema defines a minimal set of node types together with a flexible attribute mechanism. This design keeps the representation compact while allowing new operators, collectives, or system specific annotations to be added without breaking compatibility. Communication is treated as a first class node alongside computation and memory, so that both parallelization strategies and system level effects are captured in the same graph. By unifying these elements in a portable format, the schema enables performance modeling and codesign without exposing proprietary model or dataset details, and provides a foundation on which analysis tools, replayers, and simulators can build consistently.

% \begin{table}[t!]
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|c|c|c|}
%     \hline
%     \textbf{Field Name} & \textbf{Data Type} & \textbf{Description} \\ \hline
%     id                  & uint64             & Unique node ID \\ \hline
%     name                & string             & Node name \\ \hline
%     type                & enum(NodeType)     & Node category (compute, memory, comm) \\ \hline
%     ctrl\_deps          & repeated uint64    & Control dependency IDs \\ \hline
%     data\_deps          & repeated uint64    & Data dependency IDs \\ \hline
%     start\_time\_micros & uint64             & (Optional) start time hint \\ \hline
%     duration\_micros    & uint64             & (Optional) duration hint \\ \hline
%     inputs/outputs      & IOInfo             & Values, shapes, types (string encoded) \\ \hline
%     attr                & repeated AttributeProto & Extensible metadata \\ \hline
%     \end{tabular}
%     }
%     \caption{Chakra node schema.}
%     \label{tab:chakra-node-schema}
% \end{table}

% The Chakra schema defines the interface between execution traces and simulators. It is intentionally minimal in required fields yet extensible to capture diverse metadata. Each node (\autoref{tab:chakra-node-schema}) is uniquely identified by an \texttt{id}, has a human-readable \texttt{name}, and a \texttt{type} field that indicates whether it represents computation, memory access, or communication. Dependencies are captured by explicit control and data dependency lists, enabling the feeder to reconstruct the partial order. Additional metadata is stored in a repeated \texttt{AttributeProto} field, which functions as a flexible key-value mechanism. This design avoids hardcoding fields into the schema and allows attributes to evolve with new use cases.

% Additional metadata is carried in \texttt{AttributeProto}, a flexible key–value structure inspired by ONNX. Each attribute stores a name, optional documentation string, and a value drawn from a one-of set (scalars or repeated lists across numeric, string, boolean, or byte types). This extensibility allows the schema to evolve without changing the core node definition.

% This schema satisfies the design requirements outlined in \autoref{sec:chakra-schema-design-requirements}. First, it is \emph{minimal yet extensible}: the node schema captures only essential fields (ID, type, dependencies), while extensibility is provided through attributes. Second, it is \emph{expressive}: nodes can model computation, memory, and point-to-point or collective communication, with attributes encoding details such as tensor sizes, communication tags, or group information. Third, it is \emph{portable}: by keeping inputs, outputs, and attributes as string-encoded or repeated fields, traces can be collected at multiple abstraction levels and consumed by heterogeneous simulators without altering the schema.

% \begin{table}[t!]
%     \centering
%     \begin{tabular}{|c|c|c|}
%     \hline
%     \textbf{Field Name} & \textbf{Data Type}      & \textbf{Description}  \\ \hline
%     id                  & required uint64         & Node ID               \\ \hline
%     name                & required string         & Node name             \\ \hline
%     type                & required enum           & Node type             \\ \hline
%     parent              & repeated uint64         & Parent node IDs       \\ \hline
%     attribute           & repeated AttributeProto & Any additional fields \\ \hline
%     \end{tabular}
%     \caption{Chakra node schema.}
%     \label{tab:chakra-node-schema}
    
%     \begin{tabular}{|c|c|c|}
%     \hline
%     \textbf{Field Name} & \textbf{Data Type} & \textbf{Description} \\ \hline
%     name                & required string    & Name of this attribute    \\ \hline
%     type                & required enum      & Type of this attribute   \\ \hline
%     doc\_string         & required string    & Description of this attribute    \\ \hline
%     f                   & optional float     & Float value        \\ \hline
%     i                   & optional int64     & Integer value        \\ \hline
%     s                   & optional string    & String value  \\ \hline
%     floats              & repeated float     & Repeated float values          \\ \hline
%     ints                & repeated int64     & Repeated integer values     \\ \hline
%     strings             & repeated string    & Repeated string values  \\ \hline
%     \end{tabular}
%     \caption{Chakra AttributeProto schema. \ju{Seems not important.}}
%     \label{tab:chakra-attributeproto-schema}
% \end{table}


% \ju{Update this section to have the most recent schema.}

% This subsection provides an in-depth look at the Chakra schema, which is presented in \autoref{tab:chakra-node-schema} and \autoref{tab:chakra-attributeproto-schema}. \autoref{tab:chakra-node-schema} outlines the Chakra node schema, while \autoref{tab:chakra-attributeproto-schema} presents the AttributeProto schema. During the design phase, we aimed to create a schema with minimal required fields while making it highly extensible. As demonstrated in \autoref{tab:chakra-node-schema}, the schema only requires a few fields to represent a node, such as id, name, type, parent, and attribute. The id field is used to uniquely identify a node, while the name field is used for naming nodes. 
% The nodes in Chakra currently represent compute, memory and communication/networking operations.
% The type field, defined as an enum, can be one of the following: INVALID, MEM\_LOAD, MEM\_STORE, COMP, COMM\_SEND, COMM\_RECV, or COMM\_COLL\footnote{SEND and RECV are used for pt-to-pt messages, while COLL for collective messages.}. 
% INVALID works as an initial value of the type field, and it is used to ignore non-critical nodes. Memory types are used for tracing and modeling memory systems, and communication types are used for network systems. All additional metadata to model computation, memory access, and network are encoded in the attribute field. The parent field is a repeated field that holds the IDs of parent nodes to encode dependencies between nodes. Finally, the attribute field is a repeated field that significantly improves the schema's extensibility. This idea was inspired by the ONNX schema. \autoref{tab:chakra-attributeproto-schema} shows the schema for AttributeProto, which is essentially a key-value pair. AttributeProto supports six data types that can be identified using the type field: float, int, string, and their repetitions. It should be emphasized that this schema satisfies all of the requirements introduced in \autoref{sec:chakra-schema-design-requirements}.

% Note that this schema satisfies all of the requirements introduced in \autoref{sec:chakra-schema-design-requirements}. First, the schema is designed to be minimal and extensible. The Chakra node schema has critical fields such as id, name, type, parent, and attribute. All other fields can be presented as in the attribute field. However, this design necessitates complex execution trace collection and parsing codes to read and interpret all attribute fields. Second, the schema can model the performance of ML execution. As the type field suggests, nodes in a trace represent memory access, computation, and communication. Their dependencies are presented with the parent field, and various compute engines and networks can be modeled by adding more metadata in the attribute field. Third, the schema can present traces collected at any level because the attribute field is extensible.

% \subsection{Discussion}
\subsection{Design Choices}
This subsection delves into the design choices made and their associated implications.

\subsubsection{Pre-execution vs. post-execution}
Determining the appropriate level for trace collection is a crucial design choice. Generally, trace collection levels can be classified as either pre-execution or post-execution. Pre-execution refers to a stage where an ML model has not yet been explicitly optimized or tied to specific system configurations, such as compute engine type, memory bandwidth, or network topology. Collecting a trace at the pre-execution stage allows for performance projection across various systems, as it is not tethered to a particular configuration. Conversely, the post-execution stage involves optimizing and executing the ML model on an actual system. Traces gathered during this stage are tightly linked to the real system on which the model is run. Although these traces accurately represent real-world phenomena, their utility for performance projection is limited due to the varying optimization and parallelization strategies required by different systems. The Chakra schema is designed to accommodate any execution stage. However, how to collect traces from a real system without being tightly bound to it remains an open question.

\subsubsection{Execution graphs vs. Execution traces}
Execution graphs and execution traces are closely related concepts, both represented as graphs, but they serve distinct purposes. Execution graphs are designed to capture precise model structure and execution semantics within frameworks such as PyTorch~\cite{pytorch}, TensorFlow~\cite{tensorflow}, and ONNX~\cite{onnx_github}, and are primarily used for correctness and optimization of training. Execution traces, in contrast, abstract away framework details and focus on replay, simulation, and emulation in order to assess performance and scalability in a framework-agnostic manner. 

Chakra provides a standardized schema that can encode both forms, enabling execution graphs to be translated into traces and shared in a portable representation. 
This unification allows organizations to exchange execution information safely and for downstream tools such as replayers and simulators to consume it without framework-specific adapters.

\subsubsection{Multi-node representation}
In the current Chakra implementation, each NPU maintains its own execution trace. With $N$ NPUs, $N$ distinct traces are generated. This design simplifies collection and replay since each NPU records only its local activity without referencing the execution of others. However, this per-device isolation reduces the opportunity for global scheduling, where work could be reassigned or balanced across NPUs. The Chakra schema does not prohibit such an approach, but its default mode of operation assumes per-device traces.

To support collective communication and parallelism across devices, Chakra uses a concept similar to \emph{Process Groups} in PyTorch. In PyTorch, a Process Group defines a set of ranks that participate in a collective operation such as \texttt{all\_reduce}, \texttt{all\_gather}, or \texttt{reduce\_scatter}. Chakra encodes the same idea by attaching a group identifier to communication nodes. This makes it possible to represent communication patterns over arbitrary subsets of NPUs. In practice, this allows traces to describe combinations of tensor, pipeline, data, and expert parallelism without altering the schema.

Through Process Groups, Chakra can represent complex parallelization and communication strategies in a uniform way, while keeping the schema itself minimal and device traces independent.
